Learning Samples Importance: Parameterizing Dual Variables in Everywhere Learning

Everywhere learning provides a principled framework for training AI models under constraints that must hold throughout the data distribution. In the dual domain, these pointwise constraints give rise to functional dual variables. In this work, we propose to learn these dual variables, motivated by the fact that their values encode useful information about the underlying constrained problem. By representing the dual variable as a parametric function of each sample, we enable the learned multiplier to be evaluated on new, unseen samples. This contrasts with standard empirical dual formulations, which assign an independent multiplier to each training sample. We characterize the error in the recovered primal solution induced by restricting the dual variable to a parametric function class and show that it is controlled by how well this class approximates the optimal statistical multiplier. Moreover, we show that the learned parametric multiplier retains the sensitivity interpretation of the optimal statistical multiplier, yielding approximate sensitivity guarantees that extend beyond the samples used for training. We empirically validate our theory across a variety of everywhere learning tasks, showing that the resulting constrained problems can be solved efficiently and that the learned dual variables provide meaningful representations of sample-level sensitivity.

==> 02_problem_formulation/c_apps.tex <==
\subsection{Applications}


\noindent
\textbf{Physical Systems.}
Physical systems require predictions not only to perform well on average, but must also satisfy operational requirements.
%
A representative example is the optimal power flow problem, where the model predicts a generation dispatch from the demand.
%
We promote economic operation by minimizing an expected cost loss \(\ell_{\mathrm C}\), while feasibility is imposed by requiring satisfaction of the power-flow equations and the operational limits of power-system components.
%
\begin{equation}\label{eq:physical_systems}
\begin{aligned}
\min_{f_\theta \in \mathcal H} \quad
& \mathbb E_{d\sim\mathcal D_{\mathrm P}}
\left[
\ell_{\mathrm C}\big(f_\theta(d),d\big)
\right] \\
\mathrm{s.t.} \quad
& \ell_{\mathrm{PF}}\big(f_\theta(d),d\big) \leq \epsilon_{\mathrm{PF}},
\qquad d \sim \mathcal D_{\mathrm P}\text{-a.e.}, \\
& \ell_{\mathrm{LIM}}\big(f_\theta(d),d\big) \leq \epsilon_{\mathrm{LIM}},
\qquad d \sim \mathcal D_{\mathrm P}\text{-a.e.}
\end{aligned}
\end{equation}
%
Here, the dual variables identify operating conditions whose feasibility constraints most strongly affect the solution, helping reveal stressed regimes and prioritize data collection toward operating conditions that are most informative or require closer evaluation.

\noindent
\textbf{Unlearning.}
Unlearning in language models aims to remove specific harmful or private knowledge from the model while preserving its general performance.
%
We  preserve performance by minimizing the KL divergence against the reference model over a retention dataset $D_{\mathrm R}$.
%
Unlearning is enforced by requiring the probability of undesired responses \(y_u\) to remain within prescribed bounds. The upper bound limits knowledge retention, while the lower bound prevents revealing which responses were targeted during unlearning.
%
\begin{equation}\label{eq:unlearning}
\begin{aligned}
\min_{\pi_\theta \in \mathcal H} \quad
& \mathbb E_{x_h\sim\mathcal D_{\mathrm R}}
\left[
D_{\mathrm{KL}}\!\left(
\pi_\theta(\cdot \mid x_h)
\,\middle\|\,
\pi_{\mathrm{ref}}(\cdot \mid x_h)
\right)
\right] \\
\mathrm{s.t.} \quad
& \epsilon^- \leq \pi_\theta(y_u\mid x_u) \leq \epsilon^+,
\qquad
(x_u,y_u) \sim \mathcal D_{\mathrm U}\text{-a.e.}
\end{aligned}
\end{equation}
%
The optimal multipliers identify facts or groups of facts whose unlearning constraints have the largest influence on the solution, revealing which targeted knowledge will most strongly affect the model during the unlearning process.

\noindent
\textbf{Reliability.}
A reliable model should provide consistent performance across samples. Minimizing expected risk alone does not ensure this behavior.
%
We promote overall predictive performance by minimizing the expected loss, while imposing reliability by requiring each individual loss to remain below a prescribed threshold $\epsilon$.
%
\begin{equation}\label{eq:reliability}
\begin{aligned}
\min_{f_\theta \in \mathcal H} \quad
& \mathbb E_{(x,y)\sim\mathcal D_0}
\left[
\ell_0(f_\theta(x),y)
\right] \\
\mathrm{s.t.} \quad
& \ell_0(f_\theta(x),y) \leq \epsilon,
\qquad
(x,y) \sim \mathcal D_0 \text{-a.e.}
\end{aligned}
\end{equation}
%
The optimal dual variables identify samples whose reliability constraints most strongly influence the learned predictor, providing a natural criterion for prioritizing new training data, like in continual-learning settings.




